Automated Ransomware Behavior Analysis: Pattern Extraction and Early Detection

Security operation centers (SOCs) typically use a variety of tools to collect large volumes of host logs for detection and forensic of intrusions. Our experience, supported by recent user studies on SOC operators, indicates that operators spend ample time (e.g., hundreds of man-hours) on investigations into logs seeking adversarial actions. Similarly, reconfiguration of tools to adapt detectors for future similar attacks is commonplace upon gaining novel insights (e.g., through internal investigation or shared indicators). This paper presents an automated malware pattern-extraction and early detection tool, testing three machine learning approaches: TF-IDF (term frequency-inverse document frequency), Fisher's LDA (linear discriminant analysis) and ET (extra trees/extremely randomized trees) that can (1) analyze freshly discovered malware samples in sandboxes and generate dynamic analysis reports (host logs); (2) automatically extract the sequence of events induced by malware given a large volume of ambient (un-attacked) host logs, and the relatively few logs from hosts that are infected with potentially polymorphic malware; (3) rank the most discriminating features (unique patterns) of malware and from the learned behavior detect malicious activity; and (4) allows operators to visualize the discriminating features and their correlations to facilitate malware forensic efforts. To validate the accuracy and efficiency of our tool, we design three experiments and test seven ransomware attacks (i.e., WannaCry, DBGer, Cerber, Defray, GandCrab, Locky, and nRansom). The experimental results show that TF-IDF is the best of the three methods to identify discriminating features, and ET is the most time-efficient and robust approach.

==> IEEE-format/50-related-work.tex <==
\section{Related Work}
\label{sec:RW}
Malware analysts usually adopt static and dynamic analysis techniques to understand its behavior and its risks.    


In \cite{cabaj2015network} and \cite{chen2017automated}, they analyze the activities performed by individual ransomware from initial footprint to the final compromise. In the work of \cite{cabaj2015network}, they analyze the network activity behavior of Cryptowall ransomware using HoneyPot and an automatic run-time malware analytical system called Maltester. They showed the step by step procedure that the ransomware follows from the initial footprint to the complete compromise of the system. Similarly, \cite{chen2017automated} introduce a method to identify the most discriminating features of Wannacry ransomware from a different distribution of ambient and infected logs which are collected using Cuckoo Sandbox. Their approach was also able to detect the polymorphic behavior of the ransomware, which was failed by all existing AV at that time. Though their study is limited to the analysis of only one ransomware. On the other hand, our work is a comprehensive work that analyzes and detect 7 recent ransomware in an automated way. We also present a generalized technique to detect recent ransomware.  



